Towards Just-Enough Documentation for Agile Effort Estimation: What Information Should Be Documented?

Effort estimation is an integral part of activities planning in Agile iterative development. An Agile team estimates the effort of a task based on the available information which is usually conveyed through documentation. However, as documentation has a lower priority in Agile, little is known about how documentation effort can be optimized while achieving accurate estimation. Hence, to help practitioners achieve just-enough documentation for effort estimation, we investigated the different types of documented information that practitioners considered useful for effort estimation. We conducted a survey study with 121 Agile practitioners across 25 countries. Our survey results showed that (1) despite the lower priority of documentation in Agile practices, 98% of the respondents considered documented information moderately to extremely important when estimating effort, (2) 73% of them reported that they would re-estimate a task when the documented information was changed, and (3) functional requirements, user stories, definition of done, UI wireframes, acceptance criteria, and task dependencies were ranked as the most useful types of documented information for effort estimation. Nevertheless, many respondents reported that these useful types of documented information were occasionally changing or missing. Based on our study results, we provide recommendations for agile practitioners on how effort estimation can be improved by focusing on just-enough documentation.

==> sections/Preprocess.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% RQ1-1To what extent do story points change? (#flucuate \wis{}, fluctuation size)

\subsection{Data Preprocessing}\label{sec:preprocess}

To ensure that the participants are able to answer the questionnaire based on their \textit{direct} and \textit{recent} experience of \textit{Agile effort estimation}, we report our study results based on the respondents that satisfied the following three criteria.

\begin{description}
    \item[1) The respondent must work in an Agile team.]
    We exclude respondents who did not use Agile software development methodology~\cite{stoica2013software}, i.e., the respondents that their team are using Waterfall model, Incremental model, and not sure or N/A.
    \item[2) The respondents' team must perform effort estimation.]
    We exclude respondents whose team does not estimate effort.
    The noted reasons for this were: 1) estimation give limited value for their cases (i.e., bug-fixing or refactoring) and 2) they are working in deadline-driven environment.
    \item[3) The respondents must be involved in effort estimation.]
    We exclude respondents that never participated in effort estimation of their team.
\end{description}


==> sections/RQ2.tex <==
\subsection{(RQ2) \rqii}

\begin{figure}[h!]
    \centering
%    \vspace*{-0.1in}
    \hspace*{-0.15in}
    \includegraphics[width=1\linewidth]{sections/figures/docupdate.pdf}
    \caption{The frequencies that the respondents update the documented effort after re-estimation; and update other documents when new information becomes available.}
    \label{fig:docupdate}
\end{figure}

\input{src/sections/table/table_code}

\textbf{In response to Q3 and Q4, majority of the respondents (73\% and 77\%) report that they update the documented effort after re-estimation and update other documents when new information becomes available more often than most of the time (self-rated frequency of 75\% to 100\%).}
Figure~\ref{fig:docupdate} shows the frequencies that the respondents rated themselves in updating the documented effort after re-estimation (Q3); and update documents when new information becomes available (Q4).
For Q3, we observe that 53\% ($\frac{62}{117}$) and 21\% ($\frac{24}{117}$) of the respondents update the documented effort after re-estimation with the frequency of \always{} and \most{}, respectively.
For Q4, we observe that 35\% ($\frac{41}{117}$) and 43\% ($\frac{50}{117}$) of the respondents update documents when new information becomes available with the frequency of \always{} and \most{}, respectively.
We apply the Wilcoxon signed-rank test to find whether the respondents update the documented effort (Q3) and other documents (Q4) differently.
As a result, the Wilcoxon signed-rank test shows that the distribution of the responses from Q3 and Q4 are not significantly different (\sigpvalue{}).
This indicates that the respondents tend to update the documented effort after re-estimation as frequent as they update the other document when the information becomes available.




\begin{tcolorbox}[boxsep=1pt,left=2pt,right=2pt,top=2pt,bottom=2pt]
    \textbf{Findings:} The respondents update the documented effort after re-estimation as frequent as they update the other documents when new information becomes available. 73\% of the respondents update the documented effort after re-estimation most of the time or more, while 77\% of the respondents update other document when the information is changed most of the time or more.
\end{tcolorbox}




==> sections/researchquestions.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Research Questions}\label{sec:researchquestions}
\begin{enumerate}[label=\textbf{RQ\arabic*}]
    \item \textbf{\rqi{}}\\
    \underline{Motivation}: Accurate effort estimation requires an adequate understanding of a task~\cite{jorgensen2009impact,usman2018effort,svensson2019bam, Usman2016}.
While documentation can convey the information to understand the task~\cite{hoda2012documentation, andriyani2017understanding, gralha2018evolution}, documentation has a lower priority than working software in the Agile concept~\cite{fowler2001agile}.
Hence, we set out this RQ to better understand how important the \di{} is for effort estimation in the real-world practices.

\item \textbf{\rqiii{}}\\
    \underline{Motivation}:
    When information is changed or becomes available, a task may be re-estimated~\cite{hoda2016multilevel, Bick2018}.
    While prior work reports that in Agile, \di{} can be changed anytime~\cite{kasauli2017requirements}, little is known to what degree such changes of \di{} lead to re-estimation.
    Therefore, we set out this RQ to investigate the impact of the change of \di{} on effort estimation. 
    
    
    

\item \textbf{\rqiv{}}\\
    \underline{Motivation}: Comprehensive documentation can be considered as overhead in Agile~\cite{fowler2001agile, hoda2012documentation}. 
    On the other hand, inadequate documentation can impact the understanding of a task~\cite{svensson2019bam, kasauli2017requirements}.
    Hence, just-enough and just-in-time documentation would be suitable for Agile practices~\cite{heck2017framework}.
    Yet, little is known what types of information that should be documented for effort estimation.

\end{enumerate}



==> sections/studydesign.tex <==

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section{Case Study Design}\label{sec:design}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

In this section, we present our rationale for our research questions, our project selection and data preparation approaches.

\input{sections/studydesign/researchquestions.tex}
\input{sections/studydesign/studiedprojects.tex}
\input{sections/studydesign/datapreparation.tex}




==> sections/studydesign/studiedprojects.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Studied Projects}
\label{sec:SP}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

In Agile software projects, \wis{} (e.g., Stories or Tasks) are recorded in the product backlog~\cite{sedano2019product}.
In recent practice, development teams use an online task management system (e.g., JIRA) to record the \wis{} in their product backlog ~\cite{hoda2016multilevel, Porru2016, Choetkiertikul2019}.
Each \wi{} typically includes a summary, description, estimated effort, and other details.
%Before a \wi{} will be implemented, the development team will perform a detailed analysis to acquire more clarity and completeness~\cite{sedano2019product, svensson2019bam}.
%Then, the team estimates the effort required to complete the \wis{}.
%Finally, the team prioritizes the work items and selects the work items that will be implemented in the development phase~\cite{usman2017effort, rubin2012essential}.
%Figure~\ref{fig:productbacklog} shows an overview of the product backlog analysis process.
To study the \spchgs{}, we select projects that satisfy the following criteria.

\begin{LaTeXdescription}
\item[Criterion 1 -- Traceability:] Since we will investigate the \spchgs{} (i.e., the activity of SP assignments), we need the historical data to determine whether the SP were changed.
Hence, we opt to study the projects where the activities are recorded in a task management system.

\item[Criterion 2 -- Active SP Usage:] We want to study projects that actively use SP as a unit to represent the effort required to complete a \wi{}.
Hence, we focus our study on the projects that have a relatively large proportion of \wis{} with SP.

\item[Criterion 3 -- \spchg{} policy:] Since we want to study the re-estimation practice (\spchg{}), we need to ensure that the SP changes are allowed in the project.
Hence, we select only the projects where the effort estimation practice generally allows the SP to be changed.

\end{LaTeXdescription}

To satisfy our first criterion, we obtain a list of 16 Agile software projects provided by Choetkiertikul et al.~\cite{Choetkiertikul2019}.
These 16 projects use JIRA\footnote{atlassian.com/software/jira} to track their development tasks and SP assignment activities.
Unfortunately, two of these 16 projects (i.e., JIRA Software and Mule Studio) no longer provide public access.
Hence, 14 Agile software projects are remaining.

\input{sections/table/table_project_overview.tex}

To satisfy our second criterion, we examine the proportion of the \wis{} that have SP and are marked as closed.
As shown in Table~\ref{tab:project_overview}, we find that Aptana Studio, Bamboo, Moodle, and Talend ESB do not satisfy our second criterion since only 2\%-7\% of their \wis{} have SP and are marked as closed.
After we clean the data (see Section~\ref{sec:DP}-DP2), we find that the number of \wis{} in Clover, Duracloud, and Usergrid is relatively low.
Hence, we exclude these projects from our study.

To satisfy our third criterion, we contact the core developers of the remaining seven projects to confirm whether they generally allow \spchg{} or not.
The core developers of six projects, except Talend Data Quality, confirmed that SP are generally allowed to be changed.
Hence, we exclude Talend Data Quality from our study.

Finally, \projectCount{} projects satisfied the three criteria.
Table~\ref{tab:project_overview} shows an overview of the \projectCount{} projects that we will use in this study.
Appcelerator Studio (AS) is an Integrated Development Environment (IDE) tool for web and mobile application development.\footnote{docs.axway.com/bundle/Appcelerator\_Studio\_allOS\_en}
Data Management (DM) is data management systems for storing and manipulating the data from Rubin Observatory.\footnote{lsst.org/about/dm}
Apache Mesosphere (ME) is a resource management and scheduling system for clusters.\footnote{mesos.apache.org}
Mule (MU) is an integration platform that handles communication between subsystems.\footnote{github.com/mulesoft/mule}
Titanium SDK/CLI (TI) is a Software Development Kit (SDK) that used to develop native, mobile web, and hybrid applications.\footnote{appcelerator.com/titanium/titanium-sdk/4}
Spring XD (XD) is a system used for data ingestion, real-time analytics, batch processing, and data export to ease big data application development.\footnote{projects.spring.io/spring-xd}
These projects are open-source projects.
The systems are developed and maintained by a team of developers or an organization with multiple teams.
The typical length of their development iterations is 2--4 weeks.


==> sections/table/table_di.tex <==
\begin{table}[!t]
\caption{The code.}
\label{tab:code}
\vspace*{-0.03in}
\hspace*{0.15in}
\resizebox{0.9\linewidth}{!}{
\centering
%\normalsize
\setlength\tabcolsep{2pt}
\begin{tabular}{\columnwidth}{|l|X|}
\hline

Documented Information & Description \\ \hline
User story
& A lightweight format to express the desired business value and to represent the conversation related to the task~\cite{james2010scrum,rubin2012essential}.\\ \hline

Definition of Done
& Definition of Done is a set of common conditions that applied to multiple tasks (e.g., user stories in a sprint) to be considered as done~\cite{rubin2012essential, james2010scrum}.  \\ \hline

Acceptance criteria
& A set of conditions to define the desired behavior that must be satisfied to be accepted by stakeholders~\cite{rubin2012essential, james2010scrum}.\\ \hline

\multirow{2}{*}{\begin{tabular}{@{}l@{}}Test scenarios\\or Test cases\end{tabular}}
& The formal tests to determine whether a developed task satisfies the predefined acceptance criteria or requirements~\cite{Davies2014, rubin2012essential}.  \\ \hline

\multirow{2}{*}{\begin{tabular}{@{}l@{}}Functional\\requirement\end{tabular}}
& A description of the system that should be implemented to satisfy business needs. It is often written in the form of \textit{shall} statements~\cite{lauesen2002software}.\\ \hline


\multirow{2}{*}{\begin{tabular}{@{}l@{}}Non-functional\\requirement\end{tabular}}
& A description of behavior (requirement) that does not relate to functionality but a property or characteristic that a system should have been met, e.g., reliability, efficiency, usability, maintainability, or portability.~\cite{behutiye2017non} \\ \hline

Task dependencies
& A reliance that the task has on a factor, event, or the other task outside its scope of work.~\cite{strode2012taxonomy}\\ \hline

Code examples
& A chunk of example code (or a link to an example code) to assist the implementation~\cite{Davies2014}.\\ \hline

\multirow{2}{*}{\begin{tabular}{@{}l@{}}UI wireframes or\\pre-designed UI\end{tabular}}
& Graphical design, mockups, or wireframes of user interfaces (or a link to these materials) as a guide for software development~\cite{Davies2014}. \\ \hline

API reference guide
& A document (or a link to a document) that describes the interfaces required to invoke a module or connect to another system~\cite{aghajani2019software}.  \\ \hline
\end{tabular}
}
\end{table}




\begin{table}[]
\label{tab:di}
%\vspace*{-0.08in}
%\hspace*{-0.1in}
%\centering
%\normalsize

\end{table}

